Qualifying Software Engineers Undergraduates in DevOps -- Challenges of Introducing Technical and Non-technical Concepts in a Project-oriented Course

The constant changes in the software industry, practices, and methodologies impose challenges to teaching and learning current software engineering concepts and skills. DevOps is particularly challenging because it covers technical concepts, such as pipeline automation, and non-technical ones, such as team roles and project management. The present study investigates a course setup to introduce these concepts to software engineering undergraduates. We designed the course by employing coding to associate DevOps concepts to Agile, Lean, and Open source practices and tools. We present the main aspects of this project-oriented DevOps course, with 240 students enrolled in it since its first offering in 2016. We conducted an empirical study, with both a quantitative and qualitative analysis, to evaluate this project-oriented course setup. We collected the data from the projects repository and students perceptions from a questionnaire. We mined 148 repositories (corresponding to 72 projects) and obtained 86 valid responses to the questionnaire. We also mapped the concepts which are more challenging to students learn from experience. The results evidence that first-hand experience facilitates the comprehension of DevOps concepts and enriches classes discussions. We present a set of lessons learned, which may help professors better design and conduct project-oriented courses to cover DevOps concepts.

==> bibliography.tex <==

@INPROCEEDINGS{6349510,
author={R. P. Mahapatra and N. Sharma and A. Trivedi and C. Aman},
booktitle={2012 CSI Sixth International Conference on Software Engineering (CONSEG)},
title={Adding interactive interface to E-Government systems using AIML based chatterbots},
year={2012},
volume={},
number={},
pages={1-6},
month={Sep.},}

@article{Anthopoulos2015,
author = {Anthopoulos, Leonidas and G. Reddick, Christopher and Giannakidou, Irene and Mavridis, Nikolaos},
year = {2015},
month = {08},
pages = {},
title = {Why e-government projects fail? An analysis of the Healthcare.gov website},
journal = {Government Information Quarterly},
}
@inproceedings{Falk2018,
author = {Falk, Jessica and Poulakos, Steven and Kapadia, Mubbasir and Sumner, Robert},
year = {2018},
month = {11},
pages = {141-146},
title = {PICA: Proactive Intelligent Conversational Agent for Interactive Narratives},
doi = {10.1145/3267851.3267892}
}

@article{Soler2018,
author = {S. Perez-Soler and E. Guerra and J. de Lara},
journal = {IEEE Software},
title = {Collaborative Modeling and Group Decision Making Using Chatbots in Social Networks},
year = {2018},
volume = {35},
number = {6},
pages = {48-54},
keywords={Collaborative software;Social network services;Biological system modeling;Decision making;Software engineering},
month={November/December}
}

@inproceedings{Ranoliya2017, 
author={B. R. Ranoliya and N. Raghuwanshi and S. Singh}, 
booktitle={2017 International Conference on Advances in Computing, Communications and Informatics (ICACCI)}, 
title={Chatbot for university related FAQs}, 
year={2017}, 
volume={}, 
number={}, 
pages={1525-1530}, 
ISSN={}, 
month={Sep.},}

@inproceedings{Paetzel2018,
author = {Paetzel, Maike and Kennedy, James and Castellano, Ginevra and Lehman, Jill},
year = {2018},
month = {12},
pages = {92-100},
booktitle = {International Conference on Human-Agent Interaction 2018},
title = {Incremental Acquisition and Reuse of Multimodal Affective Behaviors in a Conversational Agent}
}
@inproceedings{Nuruzzaman2018, 
author={M. Nuruzzaman and O. K. Hussain}, 
booktitle={2018 IEEE 15th International Conference on e-Business Engineering (ICEBE)}, 
title={A Survey on Chatbot Implementation in Customer Service Industry through Deep Neural Networks}, 
year={2018}, 
volume={}, 
number={}, 
pages={54-61}, 
ISSN={}, 
month={Oct},}

@inproceedings{Melissa2018,
author = {Wen, Melissa and Meirelles, Paulo and Siqueira, Rodrigo and Kon, Fabio},
year = {2018},
booktitle = {International Conference on Open Source Systems},
month = {06},
pages = {15-25},
title = {FLOSS Project Management in Government-Academia Collaboration},
isbn = {978-3-319-92374-1},
}

@article{Michaud2018, 
author={L. N. Michaud}, 
journal={IT Professional}, 
title={Observations of a New Chatbot: Drawing Conclusions from Early Interactions with Users}, 
year={2018}, 
volume={20}, 
number={5}, 
pages={40-47}, 
ISSN={1520-9202}, 
month={Sep.},}

@article{Lebeuf2018,
author = {C. Lebeuf and M. Storey and A. Zagalsky},
journal = {IEEE Software},
title = {Software Bots},
year = {2018},
volume = {35},
number = {1},
pages = {18-23},
keywords={Software development;Graphical user interfaces;Bot (Internet);Software engineering},

month={January/February}
}

@article{Vladimir2018,
  author    = {Vladimir Vlasov and
               Akela Drissner{-}Schmid and
               Alan Nichol},
  title     = {Few-Shot Generalization Across Dialogue Tasks},
  journal   = {CoRR},
  volume    = {abs/1811.11707},
  year      = {2018},
  timestamp = {Fri, 30 Nov 2018 12:44:28 +0100}
}

@article{Liu2018, 
author={B. Liu and Z. Xu and C. Sun and B. Wang and X. Wang and D. F. Wong and M. Zhang}, 
journal={IEEE/ACM Transactions on Audio, Speech, and Language Processing}, 
title={Content-Oriented User Modeling for Personalized Response Ranking in Chatbots}, 
year={2018}, 
volume={26}, 
number={1}, 
pages={122-133}, 
ISSN={2329-9290}, 
month={Jan},}

@article{Bocklisch2017,
author = {Bocklisch, Tom and Faulker, Joey and Pawlowski, Nick and Nichol, Alan},
year = {2017},
journal   = {CoRR},
month = {12},
pages = {},
title = {Rasa: Open Source Language Understanding and Dialogue Management}
}

@misc{wu2017starspace,
  abstract = {We present StarSpace, a general-purpose neural embedding model that can solve
a wide variety of problems: labeling tasks such as text classification, ranking
tasks such as information retrieval/web search, collaborative filtering-based
or content-based recommendation, embedding of multi-relational graphs, and
learning word, sentence or document level embeddings. In each case the model
works by embedding those entities comprised of discrete features and comparing
them against each other -- learning similarities dependent on the task.
Empirical results on a number of tasks show that StarSpace is highly
competitive with existing methods, whilst also being generally applicable to
new cases where those methods are not.},
  added-at = {2017-09-16T15:07:22.000+0200},
  author = {Wu, Ledell and Fisch, Adam and Chopra, Sumit and Adams, Keith and Bordes, Antoine and Weston, Jason},
  description = {StarSpace: Embed All The Things!},
  keywords = {deep_learning embedding},
  timestamp = {2017-09-16T15:07:22.000+0200},
  title = {StarSpace: Embed All The Things!},
  year = 2017
}

@article{tavanapour_automated_nodate,
	title = {Automated {Facilitation} for {Idea} {Platforms}: {Design} and {Evaluation} of a {Chatbot} {Prototype}},
	abstract = {While much prior research has shed light on how human facilitators can effectively guide people through ideation, human facilitation is hardly scalable to platform settings, such as on idea platforms. Thus, research and practice request solutions for more structured idea platform process support. This paper contributes to this need with the underlying DSR project by proposing the prototype of a chatbot for automated facilitation of the idea submission process to explore, if a chatbot is capable of facilitating humans. We derive requirements from literature, implement a chatbot prototype and train it with data from a prior Wizard-of-Oz study. We perform user tests and compare the results to the facilitation by human facilitators. This paper presents a proof-of-concept for chatbots as facilitators. Furthermore, it provides insights on how to get from Wizard-of-Oz studies to developed chatbots; the requirements and limitations of non-human facilitation; and the level of acceptance by human participants.},
	language = {en},
	journal = {Conference: Thirty Ninth International Conference on Information Systems (ICIS)},
	year = {2018},
	author = {Tavanapour, Navid and Bittner, Eva A C},
	keywords = {survey},
	pages = {9}
}

@article{Miller17,
  author    = {Alexander H. Miller and
               Will Feng and
               Adam Fisch and
               Jiasen Lu and
               Dhruv Batra and
               Antoine Bordes and
               Devi Parikh and
               Jason Weston},
  title     = {ParlAI: {A} Dialog Research Software Platform},
  journal   = {Proceedings of the 2017 Conference on Empirical Methods in Natural Language Processing: System Demonstrations },
  volume    = {abs/1705.06476},
  year      = {2017},
  timestamp = {Mon, 13 Aug 2018 16:47:16 +0200}
}

@misc{Mycroft2019,
  author = {Mycroft},
  title = {Mycroft AI Open Source Voice Assistant},
  year = 2019,
  url = {https://mycroft.ai},
  urldate = {2010-01-12}
}


@misc{TaisBot2019,
  author = {Advanced Laboratory of Production, Research, and Innovation in Software Engineering (LAPPIS/UnB)},
  title = {Tais - a FLOSS FAQ Chatbot for the Ministry of Culture},
  year = 2019,
  url = {https://github.com/lappis-unb/tais},
  urldate = {2018-01-12}
}

@misc{Botpress2019,
  author = {Botpress},
  title = {Botpress - A Chatbot Maker \& Development Framework},
  year = 2019,
  url = {https://botpress.io/},
  urldate = {2019-01-27}
}

@article{Abdalkareem2017,
 author = {Abdalkareem, Rabe and Shihab, Emad and Rilling, Juergen},
 title = {On Code Reuse from StackOverflow},
 journal = {Inf. Softw. Technol.},
 issue_date = {August 2017},
 volume = {88},
 number = {C},
 month = aug,
 year = {2017},
 issn = {0950-5849},
 pages = {148--158},
 numpages = {11},
 acmid = {3096048},
 publisher = {Butterworth-Heinemann},
 address = {Newton, MA, USA},
 keywords = {Code reuse, Mobile app, StackOverflow},
} 
@Article{Neveol2018,
author="N{\'e}v{\'e}ol, Aur{\'e}lie
and Dalianis, Hercules
and Velupillai, Sumithra
and Savova, Guergana
and Zweigenbaum, Pierre",
title="Clinical Natural Language Processing in languages other than English: opportunities and challenges",
journal="Journal of Biomedical Semantics",
year="2018",
month="Mar",
day="30",
volume="9",
number="1",
pages="12",
abstract="Natural language processing applied to clinical text or aimed at a clinical outcome has been thriving in recent years. This paper offers the first broad overview of clinical Natural Language Processing (NLP) for languages other than English. Recent studies are summarized to offer insights and outline opportunities in this area.",
issn="2041-1480",
}

@inproceedings{Gao2015,
 author = {Mingkun Gao and Wei Xu and Chris Callison-Burch},
 title = {Cost Optimization in Crowdsourcing Translation},
 booktitle = {Proceedings of the 2015 Conference of the North American Chapter of the Association for Computational Linguistics (NAACL 2015)},
 month = {June},
 year = {2015},
 address = {Denver, Colorado},
 }
 
 @book{book:{2252039},
   title =     {Open Source Systems: Enterprise Software and Solutions},
   author =    {Ioannis Stamelos, Jesus M. Gonzalez-Barahoña, Iraklis Varlamis, Dimosthenis Anagnostopoulos},
   publisher = {Springer International Publishing},
   isbn =      {978-3-319-92374-1,978-3-319-92375-8},
   year =      {2018},
   series =    {IFIP Advances in Information and Communication Technology 525},
   edition =   {1st ed.},
   volume =    {},
  }
   
   
@article{Paschali2017,
title = "Reusability of open source software across domains: A case study",
journal = "Journal of Systems and Software",
volume = "134",
pages = "211 - 227",
year = "2017",
issn = "0164-1212",
author = "Maria-Eleni Paschali and Apostolos Ampatzoglou and Stamatia Bibi and Alexander Chatzigeorgiou and Ioannis Stamelos",
keywords = "Reusability, Open source, Application domains"
}

@article{filipczyk_chapter_nodate,
	title = {Chapter 12 - {Success} and failure in improvement of knowledge delivery to customers using chatbot—result of a case study in a {Polish} {SME}},
	language = {en},
	author = {Filipczyk, B},
	keywords = {case study},
	pages = {15},
	file = {Filipczyk - Chapter 12 - Success and failure in improvement of.pdf:/home/arthur/Zotero/storage/S3XFWM62/Filipczyk - Chapter 12 - Success and failure in improvement of.pdf:application/pdf}
}

@inproceedings{lieberman_autonomous_1997,
	address = {Atlanta, Georgia, United States},
	title = {Autonomous interface agents},
	isbn = {978-0-89791-802-2},
	language = {en},
	urldate = {2019-01-25},
	booktitle = {Proceedings of the {SIGCHI} conference on {Human} factors in computing systems  - {CHI} '97},
	publisher = {ACM Press},
	author = {Lieberman, Henry},
	year = {1997},
	pages = {67--74},
	file = {Lieberman - 1997 - Autonomous interface agents.pdf:/home/arthur/Zotero/storage/RWXQTDSP/Lieberman - 1997 - Autonomous interface agents.pdf:application/pdf}
}

@article{Weizenbaum:1966:ECP:365153.365168,
 author = {Weizenbaum, Joseph},
 title = {ELIZA\&Mdash;a Computer Program for the Study of Natural Language Communication Between Man and Machine},
 journal = {Commun. ACM},
 issue_date = {Jan. 1966},
 volume = {9},
 number = {1},
 month = jan,
 year = {1966},
 issn = {0001-0782},
 pages = {36--45},
 numpages = {10},
 acmid = {365168},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{Ruben1993,
author = {Prieto-Diaz, Ruben},
year = {1993},
month = {06},
pages = {61 - 66},
title = {Status Report: Software Reusability},
volume = {10},
journal = {Software, IEEE},
doi = {10.1109/52.210605}
}

@INPROCEEDINGS{Wu2018, 
author={S. Wu and L. Chen and P. Yang and T. Ku}, 
booktitle={2018 IEEE International Conference on Information Reuse and Integration (IRI)}, 
title={Automatic Dialogue Template Synthesis for Chatbot by Story Information Extraction}, 
year={2018}, 
volume={}, 
number={}, 
pages={485-490}, 
ISSN={}, 
month={July}}


@INPROCEEDINGS{hu2018, 
author={Z. {Hu} and Y. {Song} and E. {Gehringer}}, 
booktitle={2018 IEEE/ACM 40th International Conference on Software Engineering: Software Engineering Education and Training (ICSE-SEET)}, 
title={Open-Source Software in Class: Students' Common Mistakes}, 
year={2018}, 
volume={}, 
number={}, 
pages={40-48}, 
keywords={Open source software;Education;Computer science;Software engineering;Tools;Toy manufacturing industry;Open-source software;software engineering;open source curriculum;Expertiza}, 
doi={}, 
ISSN={}, 
month={May},}

@inproceedings{Holmes:2018,
 author = {Holmes, Reid and Allen, Meghan and Craig, Michelle},
 title = {Dimensions of Experientialism for Software Engineering Education},
 booktitle = {Proceedings of the 40th International Conference on Software Engineering: Software Engineering Education and Training},
 series = {ICSE-SEET '18},
 year = {2018},
 isbn = {978-1-4503-5660-2},
 location = {Gothenburg, Sweden},
 pages = {31--39},
 numpages = {9},
 acmid = {3183380},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {capstone, experiential learning, software engineering education},
} 

@article{article:kent:2013,
author = {G. Feitelson, Dror and Frachtenberg, Eitan and L. Beck, Kent},
year = {2013},
month = {07},
pages = {8-17},
title = {Development and Deployment at Facebook},
volume = {17},
journal = {Internet Computing, IEEE}
}

@inproceedings{Pinto:2019,
 author = {Pinto, Gustavo and Ferreira, Clarice and Souza, Cleice and Steinmacher, Igor and Meirelles, Paulo},
 title = {Training Software Engineers Using Open-source Software: The Students' Perspective},
 booktitle = {Proceedings of the 41st International Conference on Software Engineering: Software Engineering Education and Training},
 series = {ICSE-SEET '19},
 year = {2019},
 location = {Montreal, Quebec, Canada},
 pages = {147--157},
 numpages = {11},
 acmid = {3339237},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {open source communities, open source software, software engineering courses},
} 

@inproceedings{Christensen:2016,
 author = {Christensen, Henrik B{\ae}rbak},
 title = {Teaching DevOps and Cloud Computing Using a Cognitive Apprenticeship and Story-Telling Approach},
 booktitle = {Proceedings of the 2016 ACM Conference on Innovation and Technology in Computer Science Education},
 series = {ITiCSE '16},
 year = {2016},
 pages = {174--179},
 numpages = {6},
 publisher = {ACM},
 address = {New York, NY, USA}
} 

@INPROCEEDINGS{Bai:2018, 
author={X. {Bai} and M. {Li} and D. {Pei} and S. {Li} and D. {Ye}}, 
booktitle={2018 IEEE/ACM 40th International Conference on Software Engineering: Software Engineering Education and Training (ICSE-SEET)}, 
title={Continuous Delivery of Personalized Assessment and Feedback in Agile Software Engineering Projects}, 
year={2018}, 
volume={}, 
number={}, 
pages={58-67}
}


@article{Nascimento2013UsingOS,
  title={Using Open Source Projects in software engineering education: A systematic mapping study},
  author={Debora Maria Coelho Nascimento and Kenia Cox and Thiago Almeida and Wendell Sampaio and Roberto Almeida Bittencourt and Rodrigo R. G. Souza and Christina von Flach G. Chavez},
  journal={2013 IEEE Frontiers in Education Conference (FIE)},
  year={2013},
  pages={1837-1843}
}

@article{Leo2019,
  title={A Survey of DevOps Concepts and Challenges},
  author={Leonardo Leite, Carla Rocha, Fabio Kon, Dejan Milojicic, and Paulo Meirelles},
  journal={ACM Compututer Survey},
  year={2019},
}



@article{carrigton2003,
  title={Teaching software design with open source software},
  author={David Carrington, Soon-Kyeong Kim},
  journal={33rd Annual Frontiers in Education, 2003. FIE 2003},
  year={2003},
}

@article{Chung:2016,
 author = {Chung, Sam and Bang, Soon},
 title = {Identifying Knowledge, Skills, and Abilities (KSA) for Devops-aware Server Side Web Application with the Grounded Theory},
 journal = {J. Comput. Sci. Coll.},
 issue_date = {October 2016},
 volume = {32},
 number = {1},
 month = oct,
 year = {2016},
 issn = {1937-4771},
 pages = {110--116},
 numpages = {7},
 acmid = {3007250},
 publisher = {Consortium for Computing Sciences in Colleges},
 address = {USA},
} 

@inproceedings{Christensen:2016,
 author = {Christensen, Henrik B{\ae}rbak},
 title = {Teaching DevOps and Cloud Computing Using a Cognitive Apprenticeship and Story-Telling Approach},
 booktitle = {Proceedings of the 2016 ACM Conference on Innovation and Technology in Computer Science Education},
 series = {ITiCSE '16},
 year = {2016},
 isbn = {978-1-4503-4231-5},
 location = {Arequipa, Peru},
 pages = {174--179},
 numpages = {6},
 acmid = {2899426},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {cloud computing, course design, devops, programming education, virtualization},
} 


@inbook{Feijter:2018,
author = {Feijter, Rico and Overbeek, Sietse and Vliet, Rob and Jagroep, Erik and Brinkkemper, Sjaak},
year = {2018},
month = {01},
pages = {244-259},
title = {DevOps Competences and Maturity for Software Producing Organizations},
isbn = {978-3-319-91703-0}
}

@INPROCEEDINGS{Pinto:2017, 
author={G. H. L. {Pinto} and F. F. {Filho} and I. {Steinmacher} and M. A. {Gerosa}}, 
booktitle={2017 IEEE 30th Conference on Software Engineering Education and Training (CSEE T)}, 
title={Training Software Engineers Using Open-Source Software: The Professors' Perspective}, 
year={2017}, 
volume={}, 
number={}, 
pages={117-121}, 
ISSN={}, 
month={Nov}}

@InProceedings{becka:2014,
author="Morgan, Becka
and Jensen, Carlos",
editor="Corral, Luis
and Sillitti, Alberto
and Succi, Giancarlo
and Vlasenko, Jelena
and Wasserman, Anthony I.",
title="Lessons Learned from Teaching Open Source Software Development",
booktitle="Open Source Software: Mobile Open Source Technologies",
year="2014",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="133--142",
isbn="978-3-642-55128-4"
}

@article{balalaie2016microservices,
  author={Armin Balalaie and Abbas Heydarnoori and Pooyan Jamshidi},
  journal={IEEE Software},
  title={Microservices Architecture Enables DevOps: Migration to a Cloud-Native Architecture},
  year={2016},
  volume={33},
  number={3},
  pages={42-52},
  publisher = {IEEE},
  note={Code: A2}
}

@inproceedings{shahin2016architecting,
 author = {Shahin, Mojtaba and Babar, Muhammad Ali and Zhu, Liming},
 title = {The Intersection of Continuous Deployment and Architecting Process: Practitioners' Perspectives},
 booktitle = {Proceedings of the 10th ACM/IEEE International Symposium on Empirical Software Engineering and Measurement},
 series = {ESEM '16},
 year = {2016},
 pages = {44:1--44:10},
 publisher = {ACM},
  note={Code: A64}
} 

inproceedings{rajkumar2016culture, 
 author={M. Rajkumar and A. K. Pole and V. S. Adige and P. Mahanta}, 
 booktitle={2016 International Conference on Advances in Computing, Communication, Automation (ICACCA)}, 
 title={DevOps culture and its impact on cloud delivery and software development}, 
 year={2016}, 
 pages={1-6},
  note={Code: I48}
}

@inproceedings{bai2018feedback,
author={X. Bai and M. Li and D. Pei and S. Li and D. Ye},
booktitle = {Proceedings of the 40th International Conference on Software Engineering: Software Engineering Education and Training},
series = {ICSE-SEET '18},
title={Continuous Delivery of Personalized Assessment and Feedback in Agile Software Engineering Projects},
year={2018},
pages={58-67},
note={Code: I818}
}

@misc{xebia2016table,
 title={The Periodic Table of {DevOps} Tools v.2 Is Here},
 author={Necco Ceresani},
 year={2016},
 note={\url{https://blog.xebialabs.com/2016/06/14/periodic-table-devops-tools-v-2/}, accessed on April 2018.}
}

@misc{stackoverflow2017earn,
  title={How Much Do Developers Earn? Find Out with the Stack Overflow Salary Calculator},
  author={Julia Silge},
  year={2017},
  note={\url{https://stackoverflow.blog/2017/09/19/much-developers-earn-find-stack-overflow-salary-calculator/}, accessed on April 2018.}
}

@book{beyer2016site,
  title={Site Reliability Engineering: How Google Runs Production Systems},
  author={Beyer, Betsy and Jones, Chris and Petoff, Jennifer and Murphy, Niall Richard},
  year={2016},
  publisher={O'Reilly Media}
}

@misc{netflix2018devops,
    title = {{How Netflix Thinks of DevOps}},
    year = {2018},
  note={\url{https://www.youtube.com/watch?v=UTKIT6STSVM}, accessed on Jun 2018.}
}

@book{kim2016handbook,
  title={The DevOps Handbook: How to Create World-Class Agility, Reliability, and Security in Technology Organizations},
  author={Gene Kim and Jez Humble and Patrick Debois and John Willis},
  year={2016},
  publisher={IT Revolution Press}
}

@inproceedings{Sadowski:2018,
title	= {Modern Code Review: A Case Study at Google},
author	= {Caitlin Sadowski and Emma Söderberg and Luke Church and Michal Sipko and Alberto Bacchelli},
year	= {2018},
booktitle	= {International Conference on Software Engineering, Software Engineering in Practice track (ICSE SEIP)}
}

@INPROCEEDINGS{Punter2003, 
author={T. {Punter} and M. {Ciolkowski} and B. {Freimut} and I. {John}}, 
booktitle={2003 International Symposium on Empirical Software Engineering, 2003. ISESE 2003. Proceedings.}, 
title={Conducting on-line surveys in software engineering}, 
year={2003}, 
volume={}, 
number={}, 
pages={80-88}, 
ISSN={}, 
month={Sep.},}

@inproceedings{Trainer:2017,
 author = {Trainer, Erik H. and Kalyanasundaram, Arun and Herbsleb, James D.},
 title = {e-Mentoring for Software Engineering: A Socio-technical Perspective},
 booktitle = {Proceedings of the 39th International Conference on Software Engineering: Software Engineering and Education Track},
 series = {ICSE-SEET '17},
 year = {2017},
 isbn = {978-1-5386-2671-9},
 location = {Buenos Aires, Argentina},
 pages = {107--116},
 numpages = {10},
 acmid = {3103045},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA},
 keywords = {e-mentoring, expressive ties, free and open-source software, instrumental ties, qualitative methods, tie content},
} 

@InProceedings{devopscv:segey2020,
author="Bobrov, Evgeny
and Bucchiarone, Antonio
and Capozucca, Alfredo
and Guelfi, Nicolas
and Mazzara, Manuel
and Masyagin, Sergey",
editor="Bruel, Jean-Michel
and Mazzara, Manuel
and Meyer, Bertrand",
title="Teaching DevOps in Academia and Industry: Reflections and Vision",
booktitle="Software Engineering Aspects of Continuous Development and New Paradigms of Software Production and Deployment",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="1--14",
}

@InProceedings{Capozucca2019,
author="Capozucca, Alfredo
and Guelfi, Nicolas
and Ries, Beno{\^i}t",
editor="Bruel, Jean-Michel
and Mazzara, Manuel
and Meyer, Bertrand",
title="Design of a (Yet Another?) DevOps Course",
booktitle="Software Engineering Aspects of Continuous Development and New Paradigms of Software Production and Deployment",
year="2019",
publisher="Springer International Publishing",
address="Cham",
pages="1--18",
isbn="978-3-030-06019-0"
}

@article{Baltes_2018,
   title={Towards a theory of software development expertise},
   ISBN={9781450355735},
   url={http://dx.doi.org/10.1145/3236024.3236061},
   DOI={10.1145/3236024.3236061},
   journal={Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering - ESEC/FSE 2018},
   publisher={ACM Press},
   author={Baltes, Sebastian and Diehl, Stephan},
   year={2018}
}


@inproceedings{Tulio:2017, 
author = {Coelho, Jailton and Valente, Marco Tulio}, 
title = {Why Modern Open Source Projects Fail}, 
year = {2017},
isbn = {9781450351058},
publisher = {Association for Computing Machinery}, 
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3106237.3106246}, 
doi = {10.1145/3106237.3106246}, 
booktitle = {Proceedings of the 2017 11th Joint Meeting on Foundations of Software Engineering}, 
pages = {186–196},
numpages = {11}, 
keywords = {GitHub, Project failure, Open Source Software}, 
location = {Paderborn, Germany},
series = {ESEC/FSE 2017} }


@incollection{charmaz2008grounded,
  title={Chapter 7: Grounded Theory as an Emergent Method},
  author={Charmaz, Kathy},
  booktitle={Handbook of Emergent Methods},
  year={2008},
  publisher={The Guilford Press}
}

@article{goldman2004,
author = {Goldman, Alfredo and Kon, Fabio and Silva, Paulo and Yoder, Joseph},
year = {2004},
month = {06},
pages = {5-21},
title = {Being Extreme in the Classroom: Experiences Teaching XP.},
volume = {10},
journal = {J. Braz. Comp. Soc.},
doi = {10.1590/S0104-65002004000300002}
}

@book{SWEBOK2014,
  address = {Los Alamitos, CA},
 ition = {Version 3.0},
  editor = {Bourque, Pierre and Fairley, Richard E.},
  file = {IEEE Digital Library:2014/SWEBOK2014.pdf:PDF},
  groups = {public},
  isbn = {978-0-7695-5166-1},
  keywords = {01841 103 ieee book software engineering guide},
  publisher = {IEEE Computer Society},
  timestamp = {2018-04-16T12:18:50.000+0200},
  title = {{SWEBOK}: Guide to the Software Engineering Body of Knowledge},
  url = {http://www.swebok.org/},
  username = {flint63},
  year = 2014
}


@inproceedings{pang2020,
 author = {Candy Pang, Abram Hindle, Denilson Barbosa},
 title = {Understanding DevOps Education with Grounded Theory},
 series = {ICSE-SEET '20},
 year = {2020},
 publisher = {IEEE Press},
 address = {Piscataway, NJ, USA}
} 

@inproceedings{travassos2016SLR,
 author = {de Fran\c{c}a, Breno B. Nicolau and Jeronimo,Junior, Helvio and Travassos, Guilherme Horta},
 title = {Characterizing DevOps by Hearing Multiple Voices},
 booktitle = {Proceedings of the 30th Brazilian Symposium on Software Engineering},
 series = {SBES '16},
 year = {2016},
 location = {Maring\á, Brazil},
 pages = {53--62},
 publisher = {ACM}
} 

@book{hopper2012practicing,
  title={Practicing college learning strategies},
  author={Hopper, Carolyn H},
  year={2012},
  publisher={Cengage Learning}
}

@book{humble2010continuous,
 author = {Jez Humble and David Farley},
 title = {Continuous Delivery: Reliable Software Releases through Build, Test, and Deployment Automation}, 
 publisher = {Addison-Wesley Professional}, 
 year = {2010}
}

@misc{stackoverflow2017earn,
  title={How Much Do Developers Earn? Find Out with the Stack Overflow Salary Calculator},
  author={Julia Silge},
  year={2017},
  note={\url{https://stackoverflow.blog/2017/09/19/much-developers-earn-find-stack-overflow-salary-calculator/}, accessed on April 2018.}
}

@book{beyer2016site,
  title={Site Reliability Engineering: How Google Runs Production Systems},
  author={Beyer, Betsy and Jones, Chris and Petoff, Jennifer and Murphy, Niall Richard},
  year={2016},
  publisher={O'Reilly Media}
}


@misc{microsoft2018devops,
    author = {Donovan Brown},
    title = {{Our DevOps journey - Microsoft's internal transformation story}},
    year = {2018},
    note={DevOneConf 2018, \url{https://www.youtube.com/watch?v=cbFzojQOjyA}, accessed on Jul 2018.}
}

@misc{kelly2016better,
 title={Configuration Management And Containers: Which Is Better?},
 author={Dan Kelly},
 year={2016},
 note={\url{https://blog.containership.io/configuration-management-and-containers-which-is-better}, accessed on July 2018.}
}


@inproceedings{stol2016grounded,
  author={Klaas-Jan Stol and Paul Ralph and Brian Fitzgerald},
  booktitle={2016 IEEE/ACM 38th International Conference on Software Engineering},
  series = {ICSE '16},
  title={Grounded Theory in Software Engineering Research: A Critical Review and Guidelines},
  year={2016},
  pages={120-131}
}

@inproceedings{mulyana2018chatops,
author={Eueung Mulyana and Rifqy Hakimi and Hendrawan},
booktitle={2018 4th International Conference on Wireless and Telematics},
series = {ICWT},
title={Bringing Automation to the Classroom: A ChatOps-Based Approach},
year={2018},
pages={1--6}
}

@ARTICLE{zhu2015frequency,
author={L. Zhu and D. Xu and A. B. Tran and X. Xu and L. Bass and I. Weber and S. Dwarakanathan},
journal={IEEE Software},
title={Achieving Reliable High-Frequency Releases in Cloud Environments},
year={2015},
volume={32},
number={2},
pages={73-80},
note={Code: B12}
}

@inproceedings{dyck2015release,
author={Andrej Dyck and Ralf Penners and Horst Lichter},
booktitle={2015 IEEE/ACM 3rd International Workshop on Release Engineering},
title={Towards Definitions for Release Engineering and DevOps},
year={2015},
pages={3-3},
note={Code: B26}
}

@incollection{feijter2018maturity,
  title={{DevOps} Competences and Maturity for Software Producing Organizations},
  author={de Feijter, Rico and Overbeek, Sietse and van Vliet, Rob and Jagroep, Erik and Brinkkemper, Sjaak},
  booktitle={Enterprise, Business-Process and Information Systems Modeling},
  pages={244--259},
  year={2018},
  publisher={Springer},
  note={Code: S805}
}

@inproceedings{jari2012, 
author = {Vanhanen, Jari and Lehtinen, Timo O. A. and Lassenius, Casper}, title = {Teaching Real-World Software Engineering through a Capstone Project Course with Industrial Customers}, year = {2012}, isbn = {9781467318051}, publisher = {IEEE Press}, abstract = {In this paper, we describe how we teach real-world software engineering to students using a project course simulating in-vivo software development projects. The course gives the students an opportunity to try out in practice the skills gained on other computer science and software engineering courses. The students execute projects in teams consisting of seven to ten students, developing software for a real customer. Students spend more than 150 hours each on the project. The main stakeholders of the projects are the project team, customer, and mentor. The mentor represents the course personnel and provides practical guidance for the project team during the project. During the course, the students are supported by mentoring and experience exchange sessions. While laborious, the course is consistently ranked in the top three in the CS curriculum by the students.}, booktitle = {Proceedings of the First International Workshop on Software Engineering Education Based on Real-World Experiences}, pages = {29–32}, numpages = {4}, keywords = {industrial collaboration, capstone software project, software engineering education}, location = {Zurich, Switzerland}, series = {EduRex '12} }

@article{broman2012company,
  title={The company approach to software engineering project courses},
  author={Broman, David and Sandahl, Kristian and Baker, Mohamed Abu},
  journal={IEEE Transactions on Education},
  volume={55},
  number={4},
  pages={445--452},
  year={2012},
  publisher={IEEE}
}

@inproceedings{keefe2004using,
  title={Using Extreme Programming in a capstone project},
  author={Keefe, Karen and Dick, Martin},
  booktitle={Proceedings of the Sixth Australasian Conference on Computing Education-Volume 30},
  pages={151--160},
  year={2004}
}

@inproceedings{rong2017devopsenvy,
  title={DevOpsEnvy: an education support system for DevOps},
  author={Rong, Guoping and Gu, Shenghui and Zhang, He and Shao, Dong},
  booktitle={2017 IEEE 30th Conference on Software Engineering Education and Training (CSEE\&T)},
  pages={37--46},
  year={2017},
  organization={IEEE}
}

@inproceedings{vanhanen2012teaching,
  title={Teaching real-world software engineering through a capstone project course with industrial customers},
  author={Vanhanen, Jari and Lehtinen, Timo OA and Lassenius, Casper},
  booktitle={2012 First International Workshop on Software Engineering Education Based on Real-World Experiences (EduRex)},
  pages={29--32},
  year={2012},
  organization={IEEE}
}

==> tabs/tab_1_old.tex <==
\begin{table*}
  \caption{\devops\xspace Concepts and practices presented in the course.}
  \label{tab:commands}
  \begin{tabular}{p{3.2cm}|p{5cm}|p{4.5cm}|p{4cm}}
    %\toprule
	\hline \textbf{Categories} & \textbf{Concept} & \textbf{Practice} & \textbf{Tools} \\ \hline 
    %\midrule
    \multirow{Product Management }          & Microservice; Product quality;            & OSS Documentation standards;        & wiki; git Pages; codeclimate;        \\ 
    \multirow{ \textbf{(Process/ People)}}  & Customer satisfaction; Small features;    & unit test; review; licensing;       & coveralls; git; and SonarQube.       \\ 
                                            & Artifact management; Release engineering; & pair revision and code review;      &                                      \\
                                            & Knowledge, Skills, and Capabilities;      & architecture structure;             &                                      \\
                                            & Programing educations; Quality assurance; & product documentation; and          &                                      \\
                                            & and Artifact management.                  & pipeline stage documentation.       &                                      \\ \hline 

    %\midrule
    \multirow{Project Management}           & Risc and cost; Measurement;                & Sprint; Kanban; planing; review;    & ZenHub; HubCare; wiki;              \\
    \multirow{ \textbf{(Process/ People)}}  & People management; Short feedback cycle;  & Stand-up metting; dojos;            & Agile Visualization; Telegram;       \\
                                            & Pilots team and lead customer;            & Tasks in issues; training;          & Slack; Rocket Chat; Redmine;         \\
                                            & Compliance regulations; Team experience;  & OSS Recommended Standards;          & Google Drive; programming            \\
                                            & Aligning incentives; Breaking down silos; & Post mortem; code of contributing;  & language; and test tools.            \\
                                            & Culture of collaboration; Versioning;     & Communication in issue and PR;      &                                      \\
                                            & Sharing knowledge; Programing educations; & Full-stack and self organized teams;&                                      \\
                                            & Global community knowledge;               & git-flow; pull request; process     &                                      \\
                                            & Failure as opportunity of improvement;    & documentation; badges status        &                                      \\
                                            & Collaborate across departments;           & in readme; tracking metrics; and    &                                      \\
                                            & Knowledge, skills, and capabilities; and  & pair revision.                      &                                      \\
                                            & Artifact management.                      &                                     &                                      \\ \hline
 
    \multirow{Build Process}                & Release engineering; Continuous delivery; & Deployment pipeline stages;         & AWS Cloud Formation; Jest;           \\
    \multirow{ \textbf{(Delivery)} }        & Automation; Testing automation;           & Automation; Unit test; Integration  & Jmeter; Selenium; Sonar; Rancher;    \\
                                            & Correctness; and Static analysis;         & tests; and components tests.        & Cucumber; and Code Climate.          \\ \hline
 
    \multirow{Continuous Integration}       & Frequent and reliable release process;    & Build and deploy automated;         & Jenkins; Gitlab CI;                  \\
    \multirow{ \textbf{(Delivery)} }        & Release engineering; Deployment pipeline; & badges status in readme;            & Circle CI; and Travis.               \\
                                            & Continuous integration; Automation;       & and git-flow.                       &                                      \\
                                            & and Continuous delivery.                  &                                     &                                      \\\hline 

    \multirow{Deployment Automation}        & Frequent and reliable release process;    & Git-flow; Continuous Integration;   & Shell Script; Travis; Docker; npm;   \\
    \multirow{\textbf{(Delivery/Runtime)}}  & Release engineering; Continuous delivery; & Build and Deploy automated;         & Virtualenv; OpenStack; Vagrant;     \\
                                            & Configuration management; Automation;     & Architecture Structure;             & Kubernets; Cloud services; Chef;     \\
                                            & Infrastructure as code; Virtualization;   & Documentation; and pipline stage    & Puppet; Heroku; Flyway; Rancher;     \\
                                            & and Containerization.                     & documentation.                      & and AWS Cloud Formation.             \\\hline 

    \multirow{Monitoring \& Logging}        & You built it, you run it; Availability;   & Operation tasks in issues;          & Prometheus; Graylog; Arachni;        \\
    \multirow{ \textbf{(Delivery/Runtime)} }& After-hours support for Devs; Alerting;   & Logging; Monitoring; and            & Nagios; Zabbix; Logstash;            \\
                                            & Continuous runtime monitoring; Security;  & Benchmark.                          & Graylog; and ElasticSearch.          \\
                                            & Performance; Automation Metrics;          &                                     &                                      \\
                                            & Experiments Log management; Reliability;  &                                     &                                      \\
                                            & and Scalability Resilience.               &                                     &                                      \\%\hline  
  \end{tabular}
\end{table*}

==> tabs/table_collaboration.tex <==


\begin{table}
\caption{OSS practices overview.}
\label{tab:OssPractices}
\centering
\begin{tabular}{cc}
\textbf{OSS practices}                     & \textbf{\% of projects using} \\ \hline
\multicolumn{1}{c|}{Description}           & 85\%                          \\
\multicolumn{1}{c|}{Readme}                & 99\%                          \\
\multicolumn{1}{c|}{Code of conduct}       & 70\%                          \\
\multicolumn{1}{c|}{Contributing}          & 66\%                          \\
\multicolumn{1}{c|}{License}               & 92\%                          \\
\multicolumn{1}{c|}{Issue templates}       & 64\%                          \\
\multicolumn{1}{l|}{Pull request template} & 69\%                         
\end{tabular}

\end{table}
